3D Open-Vocabulary Panoptic Segmentation with 2D-3D Vision-Language Distillation

3D panoptic segmentation is a challenging perception task, especially in autonomous driving. It aims to predict both semantic and instance annotations for 3D points in a scene. Although prior 3D panoptic segmentation approaches have achieved great performance on closed-set benchmarks, generalizing these approaches to unseen things and unseen stuff categories remains an open problem. For unseen object categories, 2D open-vocabulary segmentation has achieved promising results that solely rely on frozen CLIP backbones and ensembling multiple classification outputs. However, we find that simply extending these 2D models to 3D does not guarantee good performance due to poor per-mask classification quality, especially for novel stuff categories. In this paper, we propose the first method to tackle 3D open-vocabulary panoptic segmentation. Our model takes advantage of the fusion between learnable LiDAR features and dense frozen vision CLIP features, using a single classification head to make predictions for both base and novel classes. To further improve the classification performance on novel classes and leverage the CLIP model, we propose two novel loss functions: object-level distillation loss and voxel-level distillation loss. Our experiments on the nuScenes and SemanticKITTI datasets show that our method outperforms the strong baseline by a large margin.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/5_limitations.tex <==
\subsection{Known Class Performance}
\label{sec:limitations}

{
\color{red}
In addition to the gap in novel class $PQ$ compared to the closed-set method, our method also experiences some (smaller) gaps for known class $PQ$. We report results for these classes on nuScenes in~\cref{table:base}. The gap is especially evident for $RQ$ for \textit{things} classes. We believe that this is likely due to two main factors. First, the closed-set P3Former sees ground truth supervision for the entire scene, while the open-set methods do not receive supervision in the ‘unknown class’ regions. Second, the introduction of the class embedding may reduce classification performance compared to fixed logit predictions. Nonetheless, our method still outperforms the PFC baseline. We will work on further bridging the gap with closed-set methods in future work.
}
